Multifractal Formalism from Large Deviations

It has often been observed that the Multifractal Formalism and the Large Deviation Principles are intimately related. In fact, Multifractal Formalism was heuristically derived using the Large Deviations ideas. In numerous examples in which the multifractal results have been rigorously established, the corresponding Large Deviation results are valid as well. Moreover, the proofs of multifractal and large deviations are remarkably similar. The natural question then is whether under which conditions multifractal formalism can be deduced from the corresponding large deviations results. More specifically, given a sequence of random variables $\{ {X_n} \}_{n\in\N}$, satisfying a Large Deviation Principle, what can be said about the multifractal nature of the level sets $K_\alpha=\{\omega: \lim_{n} \frac{X_n(\omega)}{n}=\alpha\}$. Under some technical assumptions, we establish the upper and lower bounds for multifractal spectra in terms of the large deviation rate functions, and show that many known results of multifractal formalism are covered by our setup.

==> introduction.tex <==
% !TEX root = MFviaLDP.tex

\section{Introduction}
In recent decades, researchers from the theoretical physics and mathematics communities have come across the multifractal phenomenon in order to solve certain problems. For example, in turbulence theory, it has been observed in \cite{Benzi-etc1984}-\cite{Frisch-Parisi1983} that structure functions of turbulent flows are described by multifractal sets. In \cite{Benzi-etc1984}, the authors had shown that the multifractal sets are necessary to describe the properties of various structure functions such as energy dissipation of turbulent flows. In particular, in \cite{Benzi-etc1984}, the authors proposed the random $\beta-$model by generalising the classical theory by taking into account the multifractal structure of the turbulence. Apart from these, the study of some problems in pure mathematics, such as the study of negligible sets in probability theory and ergodic theory, also led to the investigation of the multifractal spectrum of certain functions. These and other problems in physics and mathematics have been a motivation to develop a rigorous formalism of the multifractal phenomenon in a purely mathematical setting.


Start with Physics, multifractal analysis of pointwise dimensions


Natural: Multifractal analysis of other local quantities.


The similarity between the MFA and LDP results has been observed long time ago
[Physics, Riedi, Pesin]. Describe heuristic motivation using LDP.

In fact, formal similarity between the answers is not accidental.
Let us demonstrate this basic observation with the help of two well-known results.




Let us compare two old results, first LDP for Bernoulli random variables, and second, what we would now
call a multifractal result for frequencies of digits in binary expansions.
However, this result preceeds the multifractal idea by nearly 50 years.


%{\color{red} $X_i$ is bad notation}
\begin{theorem}[LDP for coin-tossing] Suppose $\left(X_k\right)$ are i.i.d. Bernoulli random variables with $\mathbb{P}\left(X_1=0\right)=\mathbb{P}\left(X_1=1\right)=$ $\frac{1}{2}$. Set $S_n=\sum_{i=1}^n X_i$, then $\{S_n/n\}$ satisfies LDP with the rate function $I(p)=\log2-H(p)$, where $H(p)=-p\log p-(1-p)\log (1-p)$ if $p\in[0,1]$, otherwise $H(p)=-\infty$. Namely,
$$
\lim_{n\to\infty} \frac{1}{n}\log {\mathbb{P}\Big(\frac{S_n}{n}\in(a,b)\Big)}=-\inf_{p\in(a,b)}I(p), \;\; \text{ for all } -\infty\leq a\leq b\leq\infty.
$$

%Then, for all $p\in \left(\frac{1}{2},1\right]$,
%$$
%\lim _{n \rightarrow \infty} \frac{1}{n} \log \mathbb{P}\left(S_n \geq p n\right)=-(\log 2 - H(p))=:-I(p),
%$$
%where $H(p)=-p\log p-(1-p)\log(1-p)$. Similarly, for all $q\in \left[0,\frac{1}{2}\right]$,
%$$
%\lim _{n \rightarrow \infty} \frac{1}{n} \log \mathbb{P}\left(S_n \leq q n\right)=-(\log 2 - H(q))=:-I(q),
%$$
%$$
%I(p)=\left\{\begin{array}{ll}
%\log 2 -H(p)& \text { if } p \in[0,1] \\
%\infty & \text { otherwise }
%\end{array}\right.\quad\text{,where } .
%$$	
\end{theorem}

%{\color{red} $\dim_H$ Hausdorff dimension}
The above theorem is one of the first Large Deviation results, and it is useful to compare it with possibly the first multifractal result by Besicovitch \cite{Besicovitch1935} and Eggleston \cite{Eggleston1949} in the 1930s and the 1940s. This multifractal result was, first, proved by Besicovitch \cite{Besicovitch1935} for $N=2$ (binary shift), and later, extended by Eggleston \cite{Eggleston1949} for general $N$ ($N$ is the cardinality of the alphabet).

%Besicovitch [1] and Eggleston [7] in the 1930s and the 1940s,
%Formula (1.4) was first proved by Besicovitch [1] for $N=2$ in 1934 (binary shift), and later for general $N$ by Eggleston [7] in 1949 .
\begin{theorem}[Besicovitch-Eggleston] Let $\Omega=\{0,1\}^{\Z_+}$, then
$$
 \operatorname{dim}_H\left\{\omega\in\Omega :\,
 \lim_n \frac 1n \sum_{j=0}^{n-1}\omega_j=p\right\}=
 \frac{H(p)}{\log 2}, \;\; \forall p\in[0,1].
 $$
%Formula (1.4) was first proved by Besicovitch [1] for $N=2$ in 1934, and later for general $N$ by Eggleston [7] in 1949 . {\bf BUT ALSO BILLINGSLEY! Ergodic Theory \& Information, 1978 [book, see Pesin-Weiss]}
	
\end{theorem}
It is important to stress that not only rate functions in the above theorems are related, but in fact, the proofs are also very similar.


%Not only the rate functions are related, the proofs of this two theorems are effectively the same.
Next to the Hausdorff dimension, there is another, but in some sense more dynamical set characteristic, known as \textit{topological entropy}, which is used frequently to analyse non-compact non-invariant sets. However, in the setting of symbolic dynamics $(\Omega:=(0,...,N-1)^{\Z_+},\sigma)$, one has $h_{\top}(\sigma,Z)=\log N\cdot dim_{H}(Z)$ for all $Z\subset \Omega$, in particular, $h_{\top}(\sigma,\Omega)=\log N$, where $\sigma:\Omega \rcirclearrowleft$ is the left shift map.
 Using the topological entropy, the previous results can be summarized as
%$$
%h_{\top}(f,K_p)= h_{\top}(f,\Omega)\cdot \dim_{H}(K_p)=H(p), \quad I(p) =h_{\top}(f,\Omega)-H(p).
%$$
%This implies that for any $p\in(0,1)$, one has
\begin{equation}\label{eq:equality1}
\fbox{$h_{\top}(\sigma,K_p)=h_{\top}(\sigma,\Omega)-I(p), \; \forall p\in\R$},
\end{equation}
where $K_{p}:=\{\omega\in\Omega:\lim_n S_n/n=p\}.$
%{\bf \color{blue} Pesin-Weiss:  since late 1990, express multifractal spectra in terms of Legendre transforms}
%
%Legendre transform,
%
%\begin{theorem}[Cramer's theorem]
%Let $\left(X_i\right)$ be i.i.d. $\mathbb{R}$-valued random variables satisfying
%$$
%\varphi(t)=\mathbb{E} e^{t X_1}<\infty \quad \forall t \in \mathbb{R} .
%$$
%Let $S_n=\sum_{i=1}^n X_i$. Then, for all $a>\mathbb{E} X_1$,
%$$
%\lim _{n \rightarrow \infty} \frac{1}{n} \log \mathbb{P}\left(S_n \geq a n\right)=-I(a),
%$$
%where
%$$
%I(z)=\sup _{t \in \mathbb{R}}[z t-\log \varphi(t)] .
%$$
%
%Clearly $\phi(t)=\frac 12(1+e^t)$, $\phi'(t) =\frac 12e^t$.
%$$\aligned
%I(z) &= \sup_{t\in\R}[ zt-\log \phi(t)]=\sup_{t\in\R}[ zt+\log 2- \log (1+e^t)]
%\\
%&=\log 2+\sup_{t\in\R}[ zt- \log (1+e^t)]
%\endaligned
%$$
%$$
%I(z) - \sup_{t\in\R}[ zt- \log (1+e^t)]=\log 2
%$$
%\end{theorem}
%
%{\bf HERE COMES A VERSION FROM PESIN -WEISS}
%
\subsection{Multifractal analysis of Birkhoff averages of H\"older continuous functions}
Most of the first results in the multifractal analysis of dynamical systems can be reduced to the the results in the multifractal analysis of Birkhoff averages of certain potentials.
%The next natural step in  the development of multifractal formalism was
%to consider Birkhoff averages of 'nice' functions.
For simplicity, suppose $\Omega=A^{\Z_+}$ is the set of all infinite
sequences $\omega=(\omega_0,\omega_1,\ldots)$ in a finite alphabet $A$, equipped with a metric $\rho$, generating the product topology. 
Denote by $\sigma:\Omega\to\Omega$ the left shift on $\Omega$. 
The \mybf{topological pressure} of a continuous function  $\phi:\Omega\to\R$ is defined as
$$
P(\phi)=\lim_{n\to\infty}\frac 1n\log
\sum_{(a_0,\ldots,a_{n-1})\in A^n}
\Bigl( \sup_{\omega\in [a_0^{n-1}]}\exp(S_n\phi(\omega))\Bigr),
\quad
S_n(\omega) =\sum_{k=0}^{n-1}\phi(\sigma^k\omega),
$$
where $[a_0^{n-1}]:=\{\omega\in\Omega: \omega_i=a_i, \;i=\overline{0,n-1}\}$ is the cylinder of the length $n$.
It is well-known that the pressure function $q\mapsto P_q(\phi):=P(q\phi)$, is convex. Moreover, by the celebrated result of D.Ruelle the pressure function for a \mybf{H\"older continuous} potential $\phi$
is \mybf{real-analytic}.

%{\color{red} This result immediately implies that the Gartner-Ellis theorem is applicable,
%and thus one has Large Deviations Principle for ergodic averages $X_n(\omega)=S_n\phi(\omega)$
%under the measure $m$ which is the measure of maximal entropy on $\Omega$.
%
%In this situation, LDP for ergodic averages $\{S_n(\omega)=\sum_{k=0}^{n-1} \phi(f^k(x))\}$ holds because of GE theorem
%
%Because the logarithmic moment generating function, defined as the limit
%$$
%\Lambda(\lambda) \triangleq \lim _{n \rightarrow \infty} \frac{1}{n} \Lambda_n(n \lambda) =P(\lambda \phi).
%$$
%exists and is real analytic.
%}

It turns out that real-analyticity of the pressure function immediately gives us the
 Large Deviations Principle for ergodic averages $X_n(\omega)=S_n\phi(\omega)$.
More specifically, one has the following result\footnote{This is not the most general form of Gartner-Ellis theorem.}
\begin{theorem}[Gartner-Ellis]\label{Gartner-Ellis}
 Suppose $\{X_n\}$ is a sequence of real-valued random variables defined
on a common probability space
$(\Omega,\mathcal F,m)$. Assume that for every $q\in\R$,  the logarithmic moment generating function, defined as the limit
$$
\Lambda(q) \triangleq \lim _{n \rightarrow \infty} \frac{1}{n} \log\mathbb E_m e^{ qX_n}=
\lim _{n \rightarrow \infty} \frac{1}{n} \log\int e^{ qX_n(\omega)} m(d\omega)
$$
exists and is finite. Denote by $\Lambda^*$ the Legendre transform (convex dual) of $\Lambda$, defined by
$$
\Lambda^*(\alpha) = \sup_{q\in \mathbb R}\Bigl(\alpha q- \Lambda(q)\Bigr).
$$
Then
\begin{itemize}
\item[(a)]  for any closed set $F\subset \R$,
$$
\limsup _{n \rightarrow \infty} \frac{1}{n} \log m\left(\left\{\omega\in\Omega:\  \frac 1nX_n(\omega)\in F\right\}\right)
 \leq-\inf _{\alpha \in F} \Lambda^*(\alpha) ;
$$

\item[(b)] if, furthermore $\Lambda(q)$ is differentiable on $\R$, for any open set $G\subset\R$,
$$\liminf _{n \rightarrow \infty} \frac{1}{n} \log
m\left(\left\{\omega\in\Omega:\  \frac 1nX_n(\omega)\in G\right\}\right)
 \geq-\inf _{\alpha \in G} \Lambda^*(\alpha).
 $$
\end{itemize}
\end{theorem}
  In order to apply the Gartner-Ellis theorem to ergodic averages $X_n(\omega)=S_n\phi(\omega)$
  it is necessary to introduce the reference measure $m$.
A good choice would be the {\it uniform } or  the {\it measure of maximal entropy} for $\Omega$. Namely, let
 $N=|A|$ the number of different letters in alphabet $A$, and let $m=\rho^{\Z+}_N$ be the product of uniform measures $\rho_N$ on $A$. Then one immediately concludes that
 $$
 \Lambda_\phi(q) = P_\phi(q)-\log N= P(q\phi)-\log N.
 $$
 Therefore, for H\"older continuous functions $\phi$'s, the logarithmic moment generating function
 $\Lambda_\phi(q)$ is also
 real-analytic, and hence the Gartner-Ellis theorem is applicable. The so-called largde deviations
 rate function is then
 $$\I_\phi(\alpha)=\Lambda^*_\phi(\alpha)=\sup_{q\in\R}\Bigl[q\alpha -\Lambda_\phi(q)\Bigr]
 =\sup_{q\in\R}\Bigl[q\alpha -P_\phi(q)+\log N\Bigr]=\log N+
P^*_\phi(\alpha).
 $$ Note also that is the topological entropy of the shift map
 $\sigma$, $h_{\top}(\sigma,\Omega)=\log N$. Hence,
 $$
  \I_\phi(\alpha) =h_\top(f,\Omega)+P_\phi^*(\alpha)
 $$
 {\color{red}
Various results on the multifractal analysis of egrodic averages of 'nice' observable, we obtained in the late 1990's
 by Pesin, Weiss, Barreira Schmeling, Olsen, and others [ (Pesin \& Co 1997, Pesin\& Weiss Takens book Record THeorem 18.6, Olsen, TV 2000]. Here, is a simplified version of in the spirit of the above mentioned results.}

 \begin{theorem}\label{mfa:smooth} Suppose $\Omega=A^{\Z_+}$ and $\phi:\Omega\to\R$ is H\"older continuous.
 For $\alpha\in\R$, consider the set
 $$
 K_\alpha=\left\{\omega\in\Omega:\
 \lim_{n\to\infty} \frac 1n \sum_{k=0}^{n-1}\phi(\sigma^k\omega)=\alpha\right\}.
 $$
 Then there exist $\underline\alpha,\overline\alpha\in\R$ such that
 \begin{itemize}
 \item for every $\alpha\in (\underline\alpha,\overline\alpha)$, $K_\alpha\ne\varnothing$  and
 $$\dim_{H}(f,K_\alpha) =\frac 1{\log N}\inf_{q}\Bigl( P(q\phi)-q\alpha\Bigr)
 =-\frac 1{\log N}\sup_{q}\Bigl( q\alpha -P(q\phi)\Bigr)=-\frac{P^*_\phi(\alpha)}{\log N}.
 $$
 \item the multifractal spectrum
 $$
 \alpha\mapsto\mathcal D_\phi(\alpha):= \dim_{H}(f,K_\alpha)
 $$
  is a real-analytic function of $\alpha$ on $( \underline\alpha,\overline\alpha)$.
 \end{itemize}
 \end{theorem}

Again, if we consider the topological entropy $h_{\top}(\sigma,\cdot)$ instead of the Hausdorff dimension
$\dim_{H}(\cdot)$, taking into account, that $h_{\top}(\sigma,\Omega)=\log N$, we obtain that the large deviations rate function and the topological entropy of level sets of ergodic averages are related
$$
\I_\phi(\alpha)+h_{\top}(\sigma,K_\alpha)=h_{\top}(\sigma,\Omega).
$$
{\color{red}
The key property: for H\"older continuous function $\phi$, and any $q\in\R$, there exists a unique
equilibrium state corresponding to the potential $q\phi$. Elaborate.
}
\\

{\color{blue}{\bf describe Takens Verbitskiy} }
It was observed in [Takens-Verbitskiy-1999-CMP], that the result of Theorem \ref{mfa:smooth} can be extended to a much larger class of dynamical systems and observables $\phi$ with the key property being that for every $q\in\R$, there is a unique equilibrium
state $\mu_q$  for $q\phi$. To ensure uniqueness, one has to make two types of assumptions:
on the map $f:\Omega\to\Omega$ and the potential (observable) $\phi:\Omega\to \R$.
For example,in [Takens-Verbitskiy-1999-CMP] it was assumed that
\begin{itemize}
\item the map $f:\Omega\to\Omega$
is an \emph{expansive } homeomorphism with  \emph{specification} property
\item
the observable $\phi:\Omega\to\R$
is a continuous observable  in the \emph{Bowen class}, i.e., for all $\epsilon>0$,
$$
\sup_{d_n(\omega,\omega')<\epsilon}\Bigl| (S_n\phi)(\omega)-(S_n\phi)(\omega')\Bigr|\le K(\epsilon)<\infty
$$
where the supremum is taken over all $\omega,\omega'$ such that
$$
d_n(\omega,\omega')=\max_{k=0,\ldots,n-1} d( f^k(\omega),f^k(\omega'))<\epsilon.
$$
\end{itemize}
Under these conditions the Gartner-Elis theorem holds for ergodic sums
$X_n(\omega)=S_n\phi(\omega)$ with a
differentiable  logarithmic moment generating function
$\Lambda(q)$; the multifractal spectrum for ergodic averages is given by the Legendre transform
of the pressure function: for all $\alpha\in (\underline\alpha,\overline\alpha)$,

\textcolor{red}{$$
h_\top(f,K_\alpha) =\inf_{q}\Bigl( P(q\phi)-q\alpha\Bigr)
 =-{P^*_\phi(\alpha)}. $$}

%
%\begin{theorem} Suppose $(\Omega,d)$ is a compact metric space, $f:\Omega\to\Omega$
%is an \emph{expansive } homomorphism with the specification property. Assume \end{theorem}
%
{\bf\color{red} QUESTION: $f:\Omega\to\Omega$ is expansive+specification.
Are the function with the Bowen property DENSE in the space of continuous observables?}

{\color{red} Weaker specifications,
Generalizations almost additive , almost Bowen Sullivan-Pfister}


\subsection{Multifractal analysis of Birkhoff averages of continuous functions}
If one considers simply continuous observables $\phi:\Omega\to\R$, it is no longer true
that  there is a unique equilibrium state $\mu_q$ for the potential $q\phi$ for all $q\in\R$.
Therefore, a different approach is required.

In case of symbolic systems ($\Omega=A^{\Z_+}$, $\sigma:\Omega\to\Omega$ is  the left-shift),
the first results were obtained independently by Fan and Feng \cite{Fan1,Fan2} and Olivier \cite{Olivier1, Olivier2}. The methods are quite different: Olivier relied on the density of H\"older continuous function
in the space of all continuous functions. Fan and Feng constructed of a so-called Moran fractal.
The approach of Fan and Feng turned out to be very suitable for generalization to abstract compact spaces.
In [Takens-Verbitskiy-2003] the following variational principle for multifractal spectra has been obtained:

 \begin{theorem}\label{mfa:general}[General continuous functions, TV 2003] Suppose $f:\Omega\to\Omega$ is
 a continuous transformation of a compact metric space $(\Omega,d)$ with the specification property
 and $\phi:\Omega\to\Omega$ is a continuous observable.
 Then there exist $\underline\alpha,\overline\alpha\in\R$ such that
for every $\alpha\in (\underline\alpha,\overline\alpha)$, $K_\alpha\ne\varnothing$,  and
 $$h_\top(f,K_\alpha) =\sup_{\mu\in\mathcal M_f(\Omega)}\Bigl\{ h_\mu(f):\quad \int \phi d\mu=\alpha\Bigr\},
 $$
 where supremum is taken over $\mathcal M_f(\Omega)$ of all $f$-invariant measures on $\Omega$, and $h_\mu(f)$ is the
 Kolmogorov-Sinai entropy of $\mu$.
 \end{theorem}

%
%For uniformly hyperbolic maps and Hölder continuous functions, Barreira and Saussol [3] established similar result as Proposition 4.7. The study of multifractal analysis for arbitrary (that is, non-Hölder) continuous functions was initiated in the symbolic dynamics setting by Olivier [38], Fan and Feng [18,19]. Similar results for maps with specification can be found in [54] (for pressure, see [55]).

For such systems, the Large Deviation Principle has been established in 1990 by Young \cite{Young}.
We will not recall the most general form of the result, but reformulate it in a such form
that the relation to the
multifractal formalism becomes apparent  immediately.


 \begin{theorem}[Theorem 1,\cite {Young}]\label{ldp:general}
 Suppose  $m$ is a not necessarily invariant  Alfors-Bowen  reference measure on $\Omega$.
Suppose $\varphi:\Omega\to \R$ continuous. Then for all $c\in \R$, one has
$$
\limsup_{n \rightarrow \infty} \frac{1}{n} \log m\left\{\frac{1}{n} S_n \varphi \ge c\right\}
\le \sup_{\mu\in\mathcal M_f(\Omega)} \left\{h_\mu(f):   \int \varphi d \mu \geq c\right\} -h_{\top}(f,\Omega).
$$
If, furthermore, $f$ has a specification property, then for all $c\in\R$, one has
$$
\liminf_{n \rightarrow \infty} \frac{1}{n} \log m\left\{\frac{1}{n} S_n \varphi >c \right\}
\ge
\sup_{\mu\in\mathcal M_f(\Omega)} \left\{h_\mu(f):   \int \varphi d \mu > c\right\} -h_{\top}(f,\Omega).
$$
\end{theorem}
This result allows us to say, that under the above conditions, the sequence of random variables $\{X_n(\omega)=(S_n\phi)(\omega)\}$ satisfies the Large Deviation Principle with the rate function
$$ I_\phi(\alpha) = h_{\top}(f,\Omega) - \sup_{\mu\in\mathcal M_f(\Omega)}\Bigl\{ h_\mu(f):\quad \int \phi d\mu=\alpha\Bigr\},
$$
As in the cases considered above, combining the results of Theorems \ref{mfa:general}  and  \ref{ldp:general}, one concludes that for topological dynamical systems with specification the large deviations rate
function and the mutlifractal spectrum are related by
$$
I_\phi(\alpha)+\mathcal E_\phi(\alpha) = h_\top(f,\Omega).
$$
% $$
%\bar{R}(\varphi, E)=\varlimsup_{n \rightarrow \infty} \frac{1}{n} \log m\left\{\frac{1}{n} S_n \varphi \in E\right\}
%\underline{R}(\varphi, E)=\underline{\lim _{n \rightarrow \infty}} \frac{1}{n} \log m\left\{\frac{1}{n} S_n \varphi \in E\right\}.
%$$
%(1) $\underline{R}(\varphi,(c, \infty)) \geq \sup \left\{h_\nu(f)-h_m(f ; \nu): \nu \in \mathscr{M}_e, \int \varphi d \nu>c\right\}$.
%(2) For $\xi \in \mathscr{V}^{+}$, we have
%$$
%\bar{R}(\varphi,[c, \infty)) \leq \sup \left\{h_\nu(f)-\int \xi d \nu: \nu \in \mathscr{M}, \int \varphi d \nu \geq c\right\} .
%$$
%(3) Assume $f$ satisfies specification (to be defined below). Then for $\xi \in$ $\mathscr{V}^{-}$, we have
%$$
%\underline{R}(\varphi,(c, \infty)) \geq \sup \left\{h_\nu(f)-\int \xi d \nu: \nu \in \mathscr{M}, \int \varphi d \nu>c\right\} .
%$$
%

 In fact, the methods  developed by Young, were instrumental in the proof of Theorem \ref{mfa:general}  in [Takens-verbitskiy-2003]



%
%
% {\color{purple}
%
%\hrule 5cm
%The natural question is the following: suppose we have a sequence of random variables $\{X_n\}$, defined on a common probability space $(\Omega,\mathcal F,\mathbb P)$, such that the Large deviation principle holds for $\{X_n\}$.
%
%
%Formulate the main idea,
%
%Formulate the main results.
%
%
%\mybf{\color{blue} Current "proof": upper bound}
%For any $q\in\R$, one has
%$$
%h_{\top}(T,K_\alpha)=-q\alpha +h_\X(T,K_\alpha,q)\le -q\alpha +h_\X(T,\Omega,q)
%$$
%by [Theorem 1, Mnotes]. Furthermore, by Theorem 2,
%$$h_\X(T, \Omega, q) \leq h_{\top}(T)+\varphi(q).
%$$
%Therefore, we can conclude that
%$$
%h_{\top}(T, K_\alpha) \leq h_{\top}(T)-q \alpha+\varphi(q),
%$$
%and hence,
%$$
%h_{\top}(T, K_\alpha) \leq h_{\top}(T)+\inf_{q}\Bigl[-q \alpha+\varphi(q)\Bigr]
%=h_{\top}(T)-\sup_{q}\Bigl[q \alpha-\varphi(q)\Bigr]=h_{\top}(T)-\varphi^*(\alpha).
%$$
%If we are able to apply Varadhan's lemma, then
%$$\varphi(q)=\lim_{n\to\infty}
%\frac{1}{n}  \log \E \left[ e^{q nX_n}\right]=
%\sup_{x \in \mathcal{X}}\{qx-I(x)\}
%$$
%
%Hence, $\varphi(q)=I^*(q)$. Thus
%$$
%h_{\top}(T, K_\alpha) \le h_{\top}(T)-\varphi^*(\alpha)= h_{\top}(T)-I^{**}(\alpha)
%$$
%In good cases, $I^{**}(\alpha)=I(\alpha)$,  and hence,
%$$
%h_{\top}(T, K_\alpha) \le h_{\top}(T)-I(\alpha).
%$$
%What do we need exactly for $I^{**}=I$? Under which conditions is the Legendre transform is self-inverse:
%convexity + compactness of level sets?
%
%The "current proof" requires 3 steps: Theorem 1, Theorem 2+ Varadhan lemma.
%Hopefully, one should have a shorter proof.
%The natural step is to eliminate the need for the extra parameter $q$, hence
%estimating the topological entropy of $K_\alpha$ directly.
%
%{\bf Step 1:} Learn \& understand the standard proof of Varadhan's lemma.
%
%{\bf Step 2:} Apply methods from the proof of Varadhan's lemma to estimate $h_{\top}(K_\alpha)$ directly.
%
%
%\begin{proof} Suppose $\{X_n\}$ satisfies the LDP with the (good) rate function $I$.
%Therefore, for any compact set $K$ one has
%$$
%\lim_{n\to\infty} \frac 1n \log\mu\left(\left\{\omega\in\Omega: \frac 1nX_n(\omega)\in K\right\}\right) =-\inf_{\alpha\in K} I(\alpha).
%$$
%\end{proof}
%}
%----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Multifractal beyond Birkhoff sums}
A number of multifractal results have been obtained for the level sets of the form
$$
K_\alpha=\Bigl\{\omega\in\Omega:\, \lim_{n\to\infty} \frac 1nX_n(\omega)=\alpha\Bigr\},
$$
where $X_n$'s are not necessarily Birkhoff sums of the form $S_n\phi$, for some $\phi$.
For example, such \emph{non-additive} observable arise naturally in the multifractal analysis of pointwise Lyapunov exponents for the products of matrices. Namely, consider a map $M:\Omega\to M_d(\R)$ is given where $M_d(\R)$ is the algebra of $d\times d$ real matrices. We can associate to every $x\in\Omega$ and $n\in\N$, a random variable $X_{n}(x):=\log||M(T^{n-1}x)M(T^{n-2}x)...M(x)||$ provided that $||M(T^{n-1}x)M(T^{n-2}x)...M(x)||\neq 0$, where $||\cdot||$ is a norm on $M_d(\R)$. Clearly, $\{X_n\}_{n\in\N}$ is not an additive sequence if $d\geq 2$.  

A non-additive sequence of potentials can also be encountered if one considers weighted ergodic sums $\{S_n^{w}f\}$ of a continuous potential $f$ on the space $\Omega$ i.e., $S_n^{w}f:=\sum_{i=0}^{n-1}w_if\circ T^i,\; n\in\Z_+$ and $w_n\in\R$ are weights \cite{Fan2021}. It is easy to see that $\{S_n^{w}f\}$ is not additive unless all the weights $w_n,\; n\in\Z_+$ are the same. 

Another example of non-additive sequences arises in studying pointwise entropies of probability measures. Suppose $\mu$ is a fully supported probability measure on $\Omega$. For a fixed $\delta>0$, define a sequence of random variables as $X_n(x):=-\log\mu (B_n(x,\delta)),\;n\in\N$, $x\in\Omega$, where $B_n(x,\delta):=\{y\in\Omega:d(T^iy, T^ix)<\delta,\;\; i=\overline{0\dots n-1}\}$, $n\geq 1$. 

We shall discuss these and other examples in greater detail in Section \ref{examples} and show how our results can be applied in these cases.
% {\color{red} PRODUCT OF MATRICES}

% Other examples, include   ratios of  Birkhoff sums
% $$
% Z_n(\omega) =\frac {(S_n\phi)(\omega)} {(S_n\psi)(\omega)}
% $$
% for strictly positive $\psi$, and the level sets of the form $\{\omega: \lim_n Z_n(\omega)\to\alpha\}$.

% AI HUA $\sum_k f_k(x_k,x_{k+1},\ldots)$

% {\color{red} MORE EXAMPLES === SAME EXAMPLES AS IN APPLICATION SECTION}

